A compact symmetric radio source born at one-tenth the current age of the Universe

Studies of high redshift radio galaxies can shed light on the activity of active galactic nuclei (AGN) in massive elliptical galaxies, and on the assembly and evolution of galaxy clusters in the Universe. J1606+3124 has been tentatively identified as a radio galaxy at a redshift of 4.56, at an era of one-tenth of the current age of the Universe. Very long baseline interferometry (VLBI) images show a compact triple structure with a size of 68 parsecs. The radio properties of J1606+3124, including the edge-brightening morphology, peaked GHz radio spectrum, slow variability, and low jet speed, consistently indicate that it is a compact symmetric object (CSO). The radio source size and expansion rate of the hotspots suggest that J1606+3124 is a young (kinematic age of ~3600 years) radio source. Infrared observations reveal a gas- and dust-rich host galaxy environment, which may hinder the growth of the jet; however, the ultra-high jet power of J1606+3124 gives it an excellent chance to grow into a large-scale double-lobe radio galaxy. If its redshift and galaxy classification can be confirmed by further optical spectroscopic observations, J1606+3124 will be the highest redshift CSO galaxy known to date.

==> tables.tex <==
% table of observation info.
\begin{table*}
	\centering
	\caption{Information about the VLBI observations of \obj}
	\label{tab:obs}
	\begin{tabular}{ccccccrccc} % four columns, alignment for each
		\hline
	
		Code & Date       & Frequency & Bandwidth & $B_\mathrm{maj}$ & $B_\mathrm{min}$ & $B_\mathrm{P.A.}$             & Peak              & $\sigma_{\rm rms}$  & Ref.   \\
		     & YYYY-MM-DD & (GHz)     & (MHz)     & (mas)            & (mas)            & \multicolumn{1}{c}{($\degr$)} & (mJy beam$^{-1}$) & (mJy beam$^{-1}$)   &        \\
	 Col.~1  &Col.~2      & Col.~3    &Col.~4     &Col.~5            &Col.~6            &Col.~7                         &Col.~8             &Col.~9               &Col.~10 \\   
		\hline
        BB023 & 1996-05-15  & 2.3 &  32  & 9.0  & 3.7  & $-$20.8 & 839.0 & 1.0 & 1 \\
        ...   & ... & 8.3 &  32  & 2.1 & 0.9 & $-18.2$ & 304.4 & 0.9 & 1 \\
        BG219e & 2014-08-09 & 2.3  & 128 & 8.2 & 4.3 & 18.8 &737.0 & 1.3&1\\
        ...   & ... & 8.7  & 384  & 2.1 & 1.1 & 20.9 & 337.0 & 0.3 & 1 \\
		BZ064B & 2017-03-19 & 8.4  & 512 & 2.5  & 0.8  & $-$1.6  & 97.9  & 0.1 & 2 \\
        UF001q & 2017-09-18 & 2.3  & 96 & 12.5 & 6.1 & $-$26.8 &763.5 & 1.0&1\\
        ...   & ... & 8.7  & 384  & 3.2 & 1.6 & $-$25.5& 323.6 & 0.9 & 1 \\
        UG002d & 2018-03-26 & 2.3  & 96 & 6.6 & 4.1 & 2.8 &685.9 & 0.9&1\\
        ...   & ... & 8.7  & 384  & 1.8 & 1.1 & 4.2 & 270.1 & 0.36 & 1 \\
		\hline
		\multicolumn{10}{p{14cm}}{\footnotesize{Notes: Col.~1 -- project code; Col.~2 -- observation date; Col.~3 -- observing frequency; Col.~4 -- bandwidth; Col.~5--7 -- major and minor axes of the synthesized beam (full width at half-maximum, FWHM) and the position angle of the major axis, measured from north to east; Col.~8 -- peak intensity in the image; Col.~9 --  root mean square (rms) noise in the image; Col.~10 -- reference to the corresponding VLBI experiment: 1--Astrogeo database; 2--this paper.}} \\
% 		\multicolumn{11}{p{14cm}}{\footnotesize{References: 1--This paper; 2--\citet{2002ApJS..141...13B}; 3--\citet{2008AJ....136..580P}; 4--Astrogeo database; 5--\citet{2018A&A...618A..68F}.}}
% 		\multicolumn{11}{p{14cm}}{\footnotesize{References: 1--\citet{2002ApJS..141...13B}; 2--\citet{2008AJ....136..580P}; 3--\citet{2018A&A...618A..68F};4--ASTROGEO; 5--This paper.}}
	\end{tabular}
\end{table*}

% table for model parameters
\begin{table*}
	\caption{Model-fitting parameters of the VLBI components.}
	\label{tab:parm}
	\begin{tabular}{ccccccccc}
		\hline
		Epoch      &Comp. &  $S_\mathrm{int}$ &  $S_\mathrm{peak}$  & $R$           &  P.A.             &  $d_\mathrm{comp}$       & $\sigma_{\rm d}$        &  $T_\mathrm{B}$\\
		(YYYY-MM-DD)&     &  (mJy) &  (mJy beam$^{-1}$)             &  (mas)        &  ($\degr$)        & (mas)                    & (mas)          & ($\times$10$^{10}$K) \\
		Col.~1     &Col.~2& Col.~3             &Col.~4              &Col.~5         &Col.~6             &Col.~7                    &Col.~8          &Col.~9                \\  
        \hline
        1996-05-15 & S   & 373$\pm$19         & 315$\pm$16          & ...           & ...               & 0.58                     & 0.01           & 10.8$\pm$0.6  \\
                   & C   & 79$\pm$4           & 70$\pm$4            & 2.49$\pm$0.01 & $-160.1\pm$0.3    & 0.39                     & 0.02           & 5.2$\pm$0.5   \\
                   & N   & 49$\pm$2           & 35$\pm$2            & 7.97$\pm$0.02 & $-162.7\pm$0.2    & 0.75                     & 0.03           & 0.84$\pm$0.08 \\
                   
        2014-08-09 & S   & 444$\pm$22         & 383$\pm$19          & ...           & ...               & 0.58                     & 0.01           & 11.7$\pm$0.8  \\
                   & C   & 99$\pm$5           & 78$\pm$4            & 2.60$\pm$0.02 & $-162.3\pm$0.6    & 0.64                     & 0.03           & 2.2$\pm$0.2   \\
                   & N   & 40$\pm$2           & 27$\pm$1            & 8.29$\pm$0.03 & $-163.0\pm$0.4    & 0.87                     & 0.07           & 0.47$\pm$0.08 \\
                   
        2017-03-19 & S   & 347$\pm$17         & 334$\pm$17          & ...           & ...               & 0.44                     & 0.02           & 17.3$\pm$1.4  \\
                   & S0  & 21$\pm$1           & 9$\pm$1             & 1.12$\pm$0.05 & $-155.2\pm$1.4    & ...                        & ...            & ...           \\
                   & C   & 81$\pm$4           & 67$\pm$3            & 2.66$\pm$0.01 & $-162.6\pm$0.6    & 0.53                     & 0.03           & 2.8$\pm$0.3   \\
                   & N   & 34$\pm$2           & 24$\pm$1            & 8.27$\pm$0.02 & $-163.7\pm$0.4    & 0.75                     & 0.06           & 0.58$\pm$0.10 \\
                   
        2017-09-18 & S   & 326$\pm$16         & 328$\pm$16          & ...           & ...               & 0.53                     & 0.01           & 10.4$\pm$0.64  \\
                   & C   & 95$\pm$5           & 63$\pm$3            & 2.49$\pm$0.02 & $-164.3\pm$0.8    & 0.61                     & 0.04           & 2.3$\pm$0.4   \\
                   & N   & 39$\pm$2           & 30$\pm$2            & 8.14$\pm$0.02 & $-163.4\pm$0.3    & 1.16                     & 0.04           & 0.26$\pm$0.02 \\
                   
        2018-03-26 & S   & 297$\pm$15         & 275$\pm$14          & ...           & ...               & 0.47                     & 0.01           & 11.9$\pm$0.7  \\
                   & S0  & 24$\pm$1           & 10$\pm$1            & 1.11$\pm$0.02 & $-177.0\pm$1.3    & ...                        & ...            & ...           \\
                   & C   & 82$\pm$4           & 71$\pm$4            & 2.63$\pm$0.01 & $-163.4\pm$0.6    & 0.57                     & 0.03           & 2.3$\pm$0.3   \\
                   & N   & 36$\pm$2           & 26$\pm$1            & 8.24$\pm$0.02 & $-163.9\pm$0.3    & 0.76                     & 0.04           & 0.56$\pm$0.07 \\ 
        \hline
        
\multicolumn{9}{p{16cm}}{\footnotesize{Notes: Col.~1 -- observing date; Col.~2 -- label of the fitted model component; Col.~3 -- peak intensity; Col.~4 -- total flux density; Col.~5 -- angular separation of the component with respect to \textcolor[rgb]{1,0,0}{S} ; Col.~6 -- position angle of the component with respect to \textcolor[rgb]{1,0,0}{S}, measured from north to east; Col.~7 -- fitted FWHM size of the circular Gaussian model component. \rev{ Note: the fit of S0 is degenerated to a point source model. }; Col.~8 -- uncertainty of $D_{\rm comp}$; Col.~9 -- brightness temperature. 
}} \\
	\end{tabular}
\end{table*}



